Thermal scanning probe lithography for fabrication of perforated metallic films

Thermal scanning probe lithography offers high resolution and versatility, making it a promising alternative for fabricating photonic devices. Here, we introduce a new method that expands its applications by enabling direct fabrication of arbitrary perforated patterns on a silver film.

==> jabbrv-all.tex <==




